RepGN:Object Detection with Relational Proposal Graph Network

Region based object detectors achieve the state-of-the-art performance, but few consider to model the relation of proposals. In this paper, we explore the idea of modeling the relationships among the proposals for object detection from the graph learning perspective. Specifically, we present relational proposal graph network (RepGN) which is defined on object proposals and the semantic and spatial relation modeled as the edge. By integrating our RepGN module into object detectors, the relation and context constraints will be introduced to the feature extraction of regions and bounding boxes regression and classification. Besides, we propose a novel graph-cut based pooling layer for hierarchical coarsening of the graph, which empowers the RepGN module to exploit the inter-regional correlation and scene description in a hierarchical manner. We perform extensive experiments on COCO object detection dataset and show promising results.

==> 1_introduction_orig.tex <==
\section{Introduction}
\label{sec:int}
 Object detection is one of the fundamental problems in computer vision. It plays an important role in many real-world applications such as image retrieval, advanced driver assistance system and video surveillance. This problem is very difficult because the object appearances vary dramatically from changes in different illuminations, view points, nonrigid deformations, poses, and the presence of occlusions. For instance, there is a large amount of partial occlusions between pedestrians standing next to each other in a crowd street and birds come in various poses and colors.

In the past few years, remarkable progress has been made to boost the performance of object detection. A common pipeline to address this problem consists of two main steps: (1) object proposal generation, (2) class-specific scoring and bounding box regression. There is a significant body of methods for generating object proposals such as \cite{carreira2012cpmc,uijlings2013selective,arbelaez2014multiscale,krahenbuhl2014geodesic,zitnick2014edge} or just a sliding window fashion \cite{felzenszwalb2010object}. Then some specific feature of the object bounding box is extracted and some classifier is applied for efficient and accurate object detection, in which the representative work includes AdaBoost algorithm \cite{viola2004robust}, DPM model \cite{felzenszwalb2010object} and deep CNN models \cite{girshick2014rich}. It has been well recognized in the vision community for years that contextual information, or \emph{relation} between objects, helps object recognition~\cite{divvala2009empirical,galleguillos2008object,torralba2003context,tu2008auto,shotton2006textonboost,mottaghi2014role,galleguillos2008object,galleguillos2010context,chen2017spatial}. Most such works are before the prevalence of deep learning. During the deep learning era, there is no significant progress about exploiting object relation for detection learning. Most methods still focus on recognizing objects separately.


One reason is that object-object relation is hard to model. The objects are at arbitrary image locations, of different scales, within different categories, and their number may vary across different images. The modern CNN based methods mostly have a simple regular network structure~\cite{he2016deep,he2017mask}. It is unclear how to accommodate above irregularities in existing methods.

Our approach is motivated by the success of graph convolutional neural network(GCN) in constructed data~\cite{britz2017massive,vaswani2017attention}. An GCN module can leverage   the corresponding information among a graph by aggregating information (or features) from a set of nodes. The aggregation weights are automatically learnt, driven by the task goal. An attention module can  model dependency between the elements, without making excessive assumptions on their locations and feature distributions. Recently, attention modules have been successfully applied in vision problems such as image captioning~\cite{xu2015show}.

In this work, for the first time we propose an graph convolutional module for object detection, whose primitive elements are object proposals.

==> 3_gcm.tex <==
\section{Graph Convolutional Module}
\label{sec:gcm}
In this section, we briefly review several GCN structures from previous works to provide some intuitions for the design of convolution on graph. Consider an undirected graph $G=(V,A)$ of $N$ nodes, where $V=\{v_i\}_{i=1}^{N}$ is the set of nodes, $A$ is a (weighted) adjacency matrix. The adjacency matrix $A \in R^{N \times N}$ records the connections between nodes, where if $v_i, v_j$ are not connected, then $A_{ij}=0$, otherwise $A_{ij} \neq 0$.
At the first place, the convolution operator at a specific node $v_j$ in graph $\mathcal{G}$ can be generally expressed as 

$$L_{conv}(j) = \sum_{i \in \mathcal{N}_{j}} w_{ij} X_i + b_j.$$
Here $X_i\in R_m$ is the input feature for node $v_i$, $b_j$ is the bias term and $w_{ij}$ is the weight which can be non-stationary and vary with respect to $j$. The set $\mathcal{N}_{j}$ defines the scope of convolution. For traditional applications, the CNN architecture is usually designed for a low-dimensional grid with the same connection pattern for every node. For example,  images can be viewed as two-dimensional grids (for each of the RGB channels, or gray scale channel), and the underlying graph $\mathcal{G}$ is formed by connecting adjacent pixels. Then $\mathcal{N}_j$ can be simply defined as a fixed-size block or window around pixel $j$.

In the more general graph settings, one can define $\mathcal{N}_j$ as the set of nodes that are adjacent to $v_j$. 
For example, the core of the fingerprint (FP) convolution operator in the work of Duvenaud et al. \cite{duvenaud2015convolutional} is to compute the average over neighbors, i.e. $w_{ij}=1$ for all $(i,j)$. With the help of adjacency matrix $A,$ we can write the operator as 
\begin{equation}
L_{FP} = AX.
\label{FP}
\end{equation}
The multiplication of $A$ and the feature matrix $X$ results in a feature averaging over neighbor nodes. One step further, the paper of node-GCN \cite{kipf2016semi} applied linear weighting and non-linear transformation in addition to the averaging:
\begin{equation}
L_{node-GCN} = \sigma(AXW).
\label{node-GCN}
\end{equation}
The weight matrix $W$ and the function $\sigma(\cdot)$ perform a linear and non-linear transformation on the feature $X$ respectively. \par




==> GCPool.tex <==

\subsection{Graph Cut Pool}

In this section, we propose a type of new pooling method aiming to get a general feature for the ground truth and help to diminish the local semantic feature difference for proposals. 

Nevertheless, some factors hinder this assumption, $1)$ unbalanced proposals, $2)$ densely distributed ground truth. 
Experiment in \cite{jiayajia} have demonstrated that the majority of negative proposals have little effect on improving performance, so it is necessary to filter easy isolated negative proposal candidates at the first time.
Also, proposals for gathered ground truths always distribute densely and are difficult to separated.
To eliminate the restrictions mentioned above, we adopt a two-step graph cut pooling approach.
Considering the proposal candidates in one image compose a graph, proposals are vertexes whereas adjoint matrix is $IoU > N_{IoU\_thr}$. 
On the first stage, we remove the connected components whose number of vertex is less than $N_{num\_thr}$ to refine the proposal candidates. 
Fig.\ref{graph_cut} (b) shows the connected components filtered. 

On the second stage, we resort to classical normalized cut algorithm \cite{norm_cut} on each connected components hoping separate proposals in one connected component into partitions. 
Fig.\ref{graph_cut} (d) shows the separated partitions by normalized cut and isolated node sets are filtered again according to step one.

After conducting graph cut hierarchically and iteratively, proposals are divided into several part and assigned pseudo labels.
Proposals with same pseudo labels comprise the $G_{i}(V_{i}, E_{i})$.
On the last but most primary stage, we conduct average graph pooling on each graph. 

\begin{equation}
    V'_{i} = \frac{1}{n}\sum_{V_{ij} \in V{i}} V_{ij} 
\label{xiaji}
\end{equation}

In Eq. \ref{xiaji}, $n$ is the number of vertex in $G_{i}$ and $V'_{i}$ is the output of the Graph Pool Layer. 

\begin{figure*}
\centering
\subfigure[]{
\includegraphics[width=0.2\textwidth]{eps/rois_connect_0_.jpg}
%\caption{fig1}
}
\quad
\subfigure[]{
\includegraphics[width=0.2\textwidth]{eps/graph_connect_0_.jpg}
}
\quad
\subfigure[]{
\includegraphics[width=0.2\textwidth]{eps/rois_cut_0_.jpg}
}
\quad
\subfigure[]{
\includegraphics[width=0.2\textwidth]{eps/graph_cut_0_.jpg}
}
\caption{(a): filtered proposals in one image;
         (b): normalized cut proposals in one image;
         (c): filtered nodes in one graph;
         (d): normalized cut nodes in one graph}
\label{graph_cut}
\end{figure*}


\subsection{Normalized Cut}
Normalized Cut(NCut)\cite{norm_cut} is a classical graph cut algorithm and designed to circumvent cutting small sets of isolated nodes in the graph by computing fraction of the total edge connections to all the nodes in the graph.

Given a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, NCut aims to divide it into $k$ disjoint sets to maximize weights of each sub-graph $A_{i}$ and minimize the weights of \textit{cut}. 

\begin{equation}
     N_{cut} = \sum_{i=0}^{k} \frac{cut(A_{i}, V/A_{i})}{assoc(A_{i}, V)}
\end{equation}

where the 
$cut(X, V) = \sum_{u \in X, v \in V} {w(u,v)}$ 
and 
$assoc(X, V) = \sum_{u \in X, t \in V} {w(u,t)}$, and $assoc(X,V)$ means the total connection from graph set $X$ to $V$. 

By minimizing the cost $N_{cut}$, $\mathcal{G}$ gets balanced partitioned and little bias. 
More details can be referred from \cite{norm_cut}.













==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> abstract.tex <==
\begin{abstract}
\label{sec:abs}
Region based object detectors achieve the state-of-the-art, but few consider to model the relation of proposals. Almost object detection frameworks rely on recognizing and localizing object instances individually. In this paper, we explore the idea of modeling the relationships among the proposals for object detection from the graph learning perspective. \par

Specifically, we present relational proposal graph network(RepGN) which is defined on object proposals and the semantic and spatial relation modeled as the edge. By integrating our RepGN module into object detectors, the relation and context constraints will be introduced to the feature extraction of regions and bounding boxes regression and classification. Furthermore, we propose a novel graph-cut based pooling layer for hierarchical coarsening of the graph, which empowers the RepGN module to exploit the inter-regional correlation and scene description in a hierarchical manner. We perform extensive experiments on COCO object detection dataset and show promising results.
\end{abstract}


With Guided Anchoring, we achieve
9:1\% higher recall on MS COCO with 90% fewer anchors
than the RPN baseline. We also adopt Guided Anchoring
in Fast R-CNN, Faster R-CNN and RetinaNet, respectively
improving the detection mAP by 2:2%, 2:7% and 1:2%. 1

==> authors.tex <==
\author{Ben Trovato}
\authornote{Both authors contributed equally to this research.}
\email{trovato@corporation.com}
\orcid{1234-5678-9012}
\author{G.K.M. Tobin}
\authornotemark[1]
\email{webmaster@marysville-ohio.com}
\affiliation{%
  \institution{Institute for Clarity in Documentation}
  \streetaddress{P.O. Box 1212}
  \city{Dublin}
  \state{Ohio}
  \postcode{43017-6221}
}

\author{Lars Th{\o}rv{\"a}ld}
\affiliation{%
  \institution{The Th{\o}rv{\"a}ld Group}
  \streetaddress{1 Th{\o}rv{\"a}ld Circle}
  \city{Hekla}
  \country{Iceland}}
\email{larst@affiliation.org}

\author{Valerie B\'eranger}
\affiliation{%
  \institution{Inria Paris-Rocquencourt}
  \city{Rocquencourt}
  \country{France}
}

\author{Aparna Patel}
\affiliation{%
 \institution{Rajiv Gandhi University}
 \streetaddress{Rono-Hills}
 \city{Doimukh}
 \state{Arunachal Pradesh}
 \country{India}}
 
\author{Huifen Chan}
\affiliation{%
  \institution{Tsinghua University}
  \streetaddress{30 Shuangqing Rd}
  \city{Haidian Qu}
  \state{Beijing Shi}
  \country{China}}

\author{Charles Palmer}
\affiliation{%
  \institution{Palmer Research Laboratories}
  \streetaddress{8600 Datapoint Drive}
  \city{San Antonio}
  \state{Texas}
  \postcode{78229}}
\email{cpalmer@prl.com}

\author{John Smith}
\affiliation{\institution{The Th{\o}rv{\"a}ld Group}}
\email{jsmith@affiliation.org}

\author{Julius P. Kumquat}
\affiliation{\institution{The Kumquat Consortium}}
\email{jpkumquat@consortium.net}

==> ccsxml.tex <==
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Understanding multimedia content~Media interpretation}
